Systematizing Modeler Experience (MX) in Model-Driven Engineering Success Stories

Modeling is often associated with complex and heavy tooling, leading to a negative perception among practitioners. However, alternative paradigms, such as everything-as-code or low-code, are gaining acceptance due to their perceived ease of use. This paper explores the dichotomy between these perceptions through the lens of ``modeler experience'' (MX). MX includes factors such as user experience, motivation, integration, collaboration \& versioning and language complexity. We examine the relationships between these factors and their impact on different modeling usage scenarios. Our findings highlight the importance of considering MX when understanding how developers interact with modeling tools and the complexities of modeling and associated tooling.

==> mapping-table.tex <==
{\footnotesize
\begin{longtable}{@{}P{1.7cm}P{2.5cm}P{1cm}P{2.5cm}P{1cm}P{2.5cm}P{1cm}P{2.5cm}P{1cm}@{}}
\caption{Mapping of the identified factors to the archetypical modelling workflows.}\label{tab:mapping-factors-workflows}\\
\toprule
\multirow{2}{*}{}                 & \multicolumn{2}{l}{\textbf{Infrastructure as Code}} & \multicolumn{2}{l}{\textbf{MBSE}}  & \multicolumn{3}{l}{\textbf{Informal Modelling}}   \\
                                  & & \textbf{Relevance} &  & \textbf{Relevance} &  & \textbf{Relevance (Informal)} & \begin{varwidth}[t]{2.5cm}\textbf{Relevance\\ (Semi-formal)}\end{varwidth}   \\
\endfirsthead
\midrule
\multicolumn{8}{l}{\textbf{Technical Factors}}\\
\midrule
Integration                       & \begin{varwidth}[t]{2.5cm}IDE integration: syntax highlighting, code completion, syntax checks, ability to deploy and test directly in the development environment\\ Process integration: supports unification of development and operations (DevOps), but does not enforce it\\ Conceptual integration: relatively direct translation of the high-level system architecture into a textual format\end{varwidth}                                                                                                                                                  & ++                 & Integration is an important aspect of using MDE in the automotive domain. Integration is related to integration into the overall system engineering process, upstream (e.g., requirement tools) and downstream tools (e.g., simulation and testing tool) including traceability between the artifacts, as well as integration of artifacts created by the OEM and/or different suppliers.                                                                                                                                                                                                              & ++                 & The main purpose of Informal modeling is to communicate ideas among humans so machines do not need to interpret the models.                                                                                                                                                                                                                                                                                                                                               & -                             & +   \\
Tool UX                           & Use of the tools in the IDE are natural for engineers since it is well-aligned with their traditional use of programming tools; perceived productivity is much higher than using the web-based interfaces provided, e.g., by AWS or MS Azure                                                                                                                                                                                                                                                                                                                      & +                  & \begin{varwidth}[t]{2.5cm}Is Integration a part of Tool UX?\\ \\ Tools are typically expert tools with a lower UX. \\ \\ There is a tendency of the ability to suffer with bad tool UX.\end{varwidth}                                                                                                                                                                                                                                                                                                                                                                                              & -/+                & It is quite important that the entrance barrier would be low, and also the quality aspects of the tools like responsiveness are very relevant, in order not to disturb the creative process.                                                                                                                                                                                                                                                                                      & +                             & +   \\
Versioning                        & Given that IaC uses a text-based notation, common versioning tools like git can be used. Inherent in the text-based format, can be done easily using highly mature tooling like git; this is also a major advantage of IaC as compared to other methods.                                                                                                                                                                                                                                                                                                          & +                  & \begin{varwidth}[t]{2.5cm}Versioning has multiple dimensions. E.g. different car series, different variants, “classical” artifact versions.\\ \\ A proper version management is mandated by standards like ASPICE.\end{varwidth}                                                                                                                                                                                                                                                                                                                                                                   & ++                 & Versioning is important as a way to store different sketches, and meta-data (e.g., author). There is also often a lot of implicit information (e.g. verbal communication) that may also need to be recorded such that sketches and their context remain interpretable later on.                                                                                                                                                                                                 & -                             & +  \\
Technical Features                & Model purpose does not require many of the more sophisticated technical features typically provided by modeling, such as analysis and simulation.                                                                                                                                                                                                                                                                                                                                                                                                                & --                 & \begin{varwidth}[t]{2.5cm}Due to the inherent complexity of the domain, the following list of technical features is incomplete. Examples of technical features are:\\ Code generation\\ \\ Simulation\\ \\ Architectural quality assurance (interface compatibility)\\ \\ Timing analysis \\ \\ Safety assessment\end{varwidth}                                                                                                                                                                                                                                                                     & ?                  & \begin{varwidth}[t]{2.5cm}Model purpose does not require a lot of the more sophisticated technical features typically provided by modeling, such as analysis and simulation. But required features depend on the level of formality of the tools.\\ Some required features in Semi-formal tools: Versioning, Collaborative modeling, Manageability, Establishing the traceability between sketches and artifacts, Navigating Sketches, Support for multiple viewpoints\end{varwidth} & -                             & ++   \\
Language Complexity               & \begin{varwidth}[t]{2.5cm}Suitable metrics to measure complexity, in this case, can be lines of code, number of files, number of concepts, control flow, documentation\\ Everything is captured in one file, some control flow for case distinctions, definition of variables\\ Documentation of the language is excellent\end{varwidth}                                                                                                                                                                                                                            & +                  & \begin{varwidth}[t]{2.5cm}Due to the inherent complexity of the domain, there exist a plethora of modeling languages to specify an architecture, behavior, tests, data structures, safety cases, etc. That results in a high number of modeling languages which are understood only by the respective subset of developers who have to collaborate to engineer the product. \\ \\ The complexity of the languages results in the high effort required for learning..\end{varwidth}                                                                                                                      & +                  & It is only relevant in the context of formal modeling. Semi-formal modeling is still only applicable to simple languages.                                                                                                                                                                                                                                                                                                                                                        & N/A                           & +   \\
Language Choice                   & \begin{varwidth}[t]{2.5cm}Here, the choice is not so much about the modeling language but mainly about the tool that manages the infrastructure. However, there are alternatives to Helm Charts (e.g., cdk8s, kustomize, Tanka) that could be selected instead. Since it is unclear how well-documented and integrated the alternatives are, this choice does influence MX.\\ Helm charts can be translated into other formats (e.g., to a Kustomize base, see https://github.com/Spazzy757/helm-to-kustomize), so vendor lock-in is not an issue.\end{varwidth} & -/+                & While there is a certain choice of languages possible, there exists standards which have to be followed, e.g., AUTOSAR. Other modeling languages like Simulink/Stateflow are industry-standards.                                                                                                                                                                                                                                                                                                                                                                                                   & --                 & It is only relevant in the context of formal modeling.                                                                                                                                                                                                                                                                                                                                                                                                                            & N/A                           & +   \\
Modeling Viewpoint                & There is only one viewpoint.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & --                 & \begin{varwidth}[t]{2.5cm}Many different viewpoints, e.g.:\\ Architectural models: AUTOSAR\\ \\ Feature Models: variant management\\ \\ Behavioral Specification: Simulink/Stateflow\\ \\ Scenario models for autonomous driving\\ \\ Digital twins (HiL)\end{varwidth}                                                                                                                                                                                                                                                                                                                            & +                  & Informal modeling is generally used in the early stages of the development process which only considers one viewpoint. The viewpoint becomes more relevant towards more formal modeling since the modeller would use different kinds of semi-formal models and use, e.g., different formalisms.                                                                                                                                                                                  & -                             & -/+  \\
System Domain                     & System domain provides computing resources in a cloud environment. The domain is clearly defined, but there are indeed several alternative solutions. This is, however, already covered in language choice and language complexity.                                                                                                                                                                                                                                                                                                                        & -/+                & System domain is clearly defined. There are not many alternatives you can use since standards and internal guidelines clearly define most aspects.                                                                                                                                                                                                                                                                                                                                                                                                                                         & N/A                & It is more relevant in the context of formal modeling, because we need to represent different abstractions related to the domain.                                                                                                                                                                                                                                                                                                                                                 & --                            & +   \\
\midrule
\multicolumn{8}{l}{\textbf{Non-technical Factors}}    \\
\midrule
Modeler-Intrinsic Motivation      & Integration, particularly the same style of tools you use as a developer, a natural workflow and ease-of-use create positive emotions. Avoids disrupting the continuity of thought. Feedback from the tooling provides immediate benefits.                                                                                                                                                                                                                                                                                                                  & ++                 & \begin{varwidth}[t]{2.5cm}While there is nearly no freedom to choose modeling languages and tools for the individual developers, the use of modeling can, e.g., improve individual productivity (e.g. codegeneration from simulink or autosar models).\\ \\ The enjoyment factor is often low.\end{varwidth}                                                                                                                                                                                                                                                                                       & -/+                & \begin{varwidth}[t]{2.5cm}Informal modeling is natural because it allows modelers to express new ideas freely and to refine them while being minimally constrained by standard notations.\\ Modeler intrinsic motivation is key, as it plays a role in both encouraging developers to do the modeling and also enhancing emotional benefits by gaining collective support.\end{varwidth}                                                                                        & ++                            & ++  \\
Organisation-Intrinsic Motivation & Integrated tooling and collaboration, as well as the possible reuse afforded by Helm, increases productivity and reduces cost. Certainty about what is deployed leads to decreased security risks.                                                                                                                                                                                                                                                                                                                                                                   & +                  & There is the tendency to consider tool usage as the “holy grail”. Buying a (modeling) tool shall solve a problem or reap benefits like improving time-to-market, reducing cost, improve quality.                                                                                                                                                                                                                                                                                                                                                                                                     & +                  & Organization intrinsic motivation is key, as it plays a role in both encouraging developers to do the modeling and also enhancing emotional benefits by bringing a shared understanding in the early stages of development.                                                                                                                                                                                                                                                       & -                             & -   \\
Organisation-Extrinsic Motivation & Tool availability is good, other external factors play a minor role.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              & -                  & Standards like ISO 26262 and ASPICE require the use of modeling.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & +                  & Extrinsic motivation is not important, because informal modeling is already highly accessible to everyone.                                                                                                                                                                                                                                                                                                                                                                        & --                            & --   \\
Social Motivation                 & There is a shared culture around infrastructure-as-code, but not necessarily for a specific tool/language. Ideally, the choice of tool would be a consensus, but it may also be driven by the choices made by most users outside of the organization.                                                                                                                                                                                                                                                                                               & -/+                & Change is difficult due to the aversion to change by the workforce structure.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & --                 & Social motivation is helpful during informal modeling because of its (typically) collaborative aspect. On the other hand, even if social motivation is lacking, informal modeling can still be expected to be practiced at some level.                                                                                                                                                                                                                                     & +                             & +   \\
Training                          & There is very little formal training on infrastructure-as-code, switching to IaC is relatively easy since it is well documented and there are a lot of examples. It is easy to acquire the necessary skills and knowledge.                                                                                                                                                                                                                                                                                                                                          & ++                 & A rather high amount of training is required to apply the tools properly.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & +                  & Training is not that important, due to the low technical barrier of using informal modeling. Semi-formal modeling requires more training.                                                                                                                                                                                                                                                                                                                                         & -                             & -/+ \\
Collaboration                     & From a technical point of view, collaboration is achieved via versioning. There is also not a lot of need to work on the infrastructure specifications collaboratively.                                                                                                                                                                                                                                                                                                                                                                                            & --                 & \begin{varwidth}[t]{2.5cm}There is collaboration inside teams, between departments, and between OEM and suppliers.\\ \\ The collaboration capabilities vary in those different collaboration scenarios. Inside teams there might be collaboration inside tools whereas the collaboration between OEM and suppliers is still often via documents and file exchange.\\ \\ Collaboration capabilities are less flexible than in “usual” software engineering, as the diversity of tools and lack of merging capabilities induces pessimistic versioning (i.e. locking of model files).\end{varwidth} & +                  & Informal modeling is about problem understanding and exchanging ideas, so collaboration would be key in this context.                                                                                                                                                                                                                                                                                                                                                             & ++                            & ++  \\

\end{longtable}}

